LiteBIRD Mission Overview after Mission Reformation

LiteBIRD is a JAXA-led space mission designed to produce all-sky microwave polarization maps. Its primary science goal is to test representative inflationary models by measuring the cosmic microwave background $B$-mode polarization generated by primordial gravitational waves, while also providing new insights into cosmology, particle physics, and astrophysics. The mission concept has been updated following the reformation activities initiated after the Mission Definition Review in 2024. The current concept preserves the central scientific objectives, while simplifying the payload configuration: a single telescope covers 12 frequency bands with band centers spanning 40 to 402~GHz, corresponding to an optical coverage of 34--448~GHz. The telescope is a cross-Dragone reflector with a 500~mm aperture diameter, cooled to approximately 5~K and coupled to transition-edge-sensor bolometer arrays operated at 0.1~K. LiteBIRD will observe from a Lissajous orbit around the Sun--Earth L2 point during a nominal 3-year survey. More specifically, the primary scientific objective is to achieve total uncertainty in the tensor-to-scalar ratio of $\delta r < 0.002$ (68\% C.L.), including contributions from foreground residuals, statistical uncertainties, instrumental systematics, and margin contingency. The corresponding map-noise requirements are specified separately for the low-, mid-, and high-frequency ranges over the reionization and recombination multipole ranges. This sensitivity makes LiteBIRD unique not only for inflationary science but also for a broad range of scientific investigations probing the history of both the early and late Universe, as well as for astrophysical processes, including Galactic science. This paper summarizes the scientific objectives, updated payload and instrument concepts, observation strategy, and ground segment plans.

==> authors_affiliations_LB_2026.12_key_spie.tex <==
% Ensure the `authblk` package is loaded:
\makeatletter
\@ifpackageloaded{authblk}{}{%
    \@ifpackageloaded{authblk-TI}{}{%
        \usepackage{authblk}% allows handling of the `_authblk.tex` file
    }%
}%
\makeatother

% The following lines handle the prepending/appending of "LiteBIRD Collaboration" for key/general/special papers:
\makeatletter
\def\@author{}
\renewcommand\@author{%
    \ifx\AB@affillist\AB@empty%
        \AB@author%
    \else%
        \ifnum\value{affil}=1%
            \def\rlap##1{##1}\Authfont{\textbf{LiteBIRD Collaboration$\mathbf{^\ast}$\\}}%
        \ifnum\value{affil}>\value{Maxaffil}%
            \def\rlap##1{##1} \AB@authlist \\*[\affilsep] \AB@affillist%
        \fi%
    \fi%
}
\makeatother

% Uncomment the following lines if you want to customize the author and affiliation fonts.
% For font types you can use: normalfont, bfseries, itshape, scshape.
% For font sizes you can use: tiny, scriptsize, footnotesize, small, normalsize, large, Large.
\renewcommand\Authfont{\normalfont\normalsize}  % normal sized normal font
\renewcommand\Affilfont{\itshape\small}         % small  sized italic font

\author[1]{K.\,Aizawa}
\author[2]{H.\,Akamatsu}
\author[1]{R.\,Akizawa}
\author[3]{E.\,Allys}
\author[4]{A.\,Anand}
\author[5]{D.\,Audley}
\author[6]{J.\,Aumont}
\author[7]{S.\,Azzoni}
\author[8,9,10]{C.\,Baccigalupi}
\author[11,12,13]{M.\,Ballardini}
\author[6]{A.\,J.\,Banday}
\author[14]{G.\,Barbieri\,Ripamonti}
\author[15]{R.\,B.\,Barreiro}
\author[16,17,18]{N.\,Bartolo}
\author[19]{S.\,Basak}
\author[20,21]{M.\,Bersanelli}
\author[22]{A.\,Besnard}
\author[23,24]{D.\,Blinov}
\author[25]{F.\,Bouchet}
\author[3]{F.\,Boulanger}
\author[20]{N.\,Brancadori}
\author[11]{T.\,Brinckmann}
\author[26]{E.\,Calabrese}
\author[12,27,28]{P.\,Campeti}
\author[8,9]{A.\,Carones}
\author[8,29,9]{F.\,Carralot}
\author[15]{F.\,J.\,Casas}
\author[15]{J.\,Chandran}
\author[2,30]{Y.\,Chinone}
\author[31]{M.\,Citran}
\author[30,14,32]{F.\,Columbro}
\author[14,32]{A.\,Coppolecchia}
\author[13]{F.\,Cuttaia}
\author[33]{P.\,Dal\,Bo}
\author[14,32]{P.\,de\,Bernardis}
\author[34,2]{T.\,de\,Haan}
\author[35]{E.\,de\,la\,Hoz}
\author[33]{M.\,De\,Lucia}
\author[14,32]{M.\,De\,Petris}
\author[36]{S.\,Della\,Torre}
\author[37]{C.\,Dickinson}
\author[27]{P.\,Diego-Palazuelos}
\author[38]{J.\,J.\,Díaz\,García}
\author[39,40]{T.\,Dotani}
\author[22]{M.\,Douspis}
\author[39]{K.\,Ebisawa}
\author[41]{H.\,K.\,Eriksen}
\author[31]{J.\,Errard}
\author[30]{E.\,Ferreira}
\author[13,42]{F.\,Finelli}
\author[20,21]{C.\,Franceschet}
\author[39]{R.\,Fujimoto}
\author[41]{U.\,Fuskeland}
\author[11,4]{G.\,Galloni}
\author[41]{M.\,Galloway}
\author[12]{M.\,Gerbino}
\author[43,36]{M.\,Gervasi}
\author[38,44]{R.\,T.\,Génova-Santos}
\author[2,30]{T.\,Ghigna}
\author[26]{S.\,Giardiello}
\author[41]{E.\,Gjerløw}
\author[25]{M.\,Gomes}
\author[13,42]{A.\,Gruppuso}
\author[45]{J.\,E.\,Gudmundsson}
\author[26]{P.\,Hargrave}
\author[37]{S.\,E.\,Harper}
\author[2,34,40]{M.\,Hasegawa}
\author[46,34]{M.\,Hazumi}
\author[47]{S.\,Henrot-Versillé}
\author[47]{L.\,T.\,Hergt}
\author[25]{E.\,Hivon}
\author[48]{K.\,Ichiki}
\author[49]{K.\,Ikuma}
\author[30]{T.\,L.\,Irikura}
\author[49,$\ast$]{H.\,Ishino}
\author[30]{B.\,Jost}
\author[50,51,52]{R.\,Keskitalo}
\author[53,39]{K.\,Kikuno}
\author[34]{K.\,Kohri}
\author[27,30]{E.\,Komatsu}
\author[14,32]{L.\,Lamagna}
\author[12]{M.\,Lattanzi}
\author[47]{C.\,Leloup}
\author[25,11]{M.\,Lembo}
\author[3]{F.\,Levrier}
\author[30]{J.\,Liu}
\author[54]{A.\,I.\,Lonappan}
\author[55,56]{M.\,López-Caniego}
\author[57]{G.\,Luzzi}
\author[58]{J.\,Macias-Perez}
\author[30]{A.\,Maeda}
\author[22]{B.\,Maffei}
\author[20]{D.\,Maino}
\author[57,14,4]{V.\,Maranchery}
\author[15]{E.\,Martínez-González}
\author[14,32]{S.\,Masi}
\author[16,17,18,59]{S.\,Matarrese}
\author[39]{F.\,T.\,Matsuda}
\author[30,39,64,$\ast$]{T.\,Matsumura}
\author[58,14]{S.\,Micheli}
\author[4,60]{M.\,Migliaccio}
\author[30]{M.\,Monelli}
\author[6]{L.\,Montier}
\author[22]{L.\,Mousset}
\author[30]{S.\,Myozen}
\author[49]{Y.\,Nagano}
\author[39]{R.\,Nagata}
\author[61]{K.\,Nagayoshi}
\author[14]{M.\,Najafi}
\author[30]{T.\,Namikawa}
\author[11,12]{P.\,Natoli}
\author[26]{F.\,Noviello}
\author[14]{A.\,Occhiuzzi}
\author[39]{K.\,Odagiri}
\author[39]{S.\,Oguri}
\author[62]{H.\,Ohsaki}
\author[63]{S.\,Okumura}
\author[11,12,22]{L.\,Pagano}
\author[14,32]{A.\,Paiella}
\author[13,42]{D.\,Paoletti}
\author[13]{S.\,Paradiso}
\author[30,15]{G.\,Pascual-Cisneros}
\author[64,65,30]{G.\,Patanchon}
\author[23,24]{V.\,Pavlidou}
\author[14,32]{F.\,Piacentini}
\author[31]{M.\,Piat}
\author[4]{G.\,Piccirilli}
\author[33]{M.\,Pinchera}
\author[14]{G.\,Pisano}
\author[57]{G.\,Polenta}
\author[66]{L.\,Porcelli}
\author[35]{F.\,S.\,Porter}
\author[27]{M.\,Reinecke}
\author[15]{M.\,Remazeilles}
\author[67,31]{A.\,Rizzieri}
\author[38,44]{J.\,A.\,Rubiño-Martín}
\author[15,68]{M.\,Ruiz-Granda}
\author[53,30]{Y.\,Sakurai}
\author[22]{L.\,Salvati}
\author[69,70]{J.\,Sanghavi}
\author[71]{G.\,Savini}
\author[72]{D.\,Scott}
\author[39,73]{Y.\,Sekimoto}
\author[74]{M.\,Shiraishi}
\author[75,33]{G.\,Signorelli}
\author[14,32]{S.\,Stellati}
\author[31]{R.\,Stompor}
\author[41]{R.\,M.\,Sullivan}
\author[73]{R.\,Takahashi}
\author[2,1,39]{R.\,Takaku}
\author[34]{H.\,Takakura}
\author[76]{Y.\,Takase}
\author[33,75]{A.\,Tartari}
\author[23,24]{K.\,Tassis}
\author[73,39]{K.\,Tateoka}
\author[13]{L.\,Terenzi}
\author[20,21]{M.\,Tomasi}
\author[47]{M.\,Tristram}
\author[39]{M.\,Tsujimoto}
\author[61]{D.\,Vaccaro}
\author[47]{L.\,Vacher}
\author[47]{B.\,van\,Tent}
\author[15]{P.\,Vielva}
\author[6]{S.\,Vinzl}
\author[39]{K.\,Watanuki}
\author[41]{D.\,J.\,Watts}
\author[41]{I.\,K.\,Wehus}
\author[67,47]{G.\,Weymann-Despres}
\author[77,71]{B.\,Winter}
\author[35]{E.\,J.\,Wollack}
\author[39]{N.\,Y.\,Yamasaki}
\author[39]{K.\,Yoshihara}
\author[78]{A.\,Zacchei}
\author[43,36]{M.\,Zannoni}
\affil[1]{The University of Tokyo, Department of Physics, Tokyo 113-0033, Japan}
\affil[2]{International Center for Quantum-field Measurement Systems for Studies of the Universe and Particles (QUP), High Energy Accelerator Research Organization (KEK), Tsukuba, Ibaraki 305-0801, Japan}
\affil[3]{Laboratoire de Physique de l’École Normale Supérieure, ENS, Université PSL, CNRS, Sorbonne Université, Université de Paris, 75005 Paris, France}
\affil[4]{Dipartimento di Fisica, Università di Roma Tor Vergata, Via della Ricerca Scientifica, 1, 00133, Roma, Italy}
\affil[5]{SRON Space Research Organization Netherlands, 9747 AD Groningen, The Netherlands}
\affil[6]{Univ Toulouse, CNES, CNRS, IRAP, Toulouse, France}
\affil[7]{Department of Astrophysical Sciences, Peyton Hall, Princeton University, Princeton, NJ, USA 08544}
\affil[8]{International School for Advanced Studies (SISSA), Via Bonomea 265, 34136, Trieste, Italy}
\affil[9]{INFN Sezione di Trieste, via Valerio 2, 34127 Trieste, Italy}
\affil[10]{IFPU, Via Beirut, 2, 34151 Grignano, Trieste, Italy}
\affil[11]{Dipartimento di Fisica e Scienze della Terra, Università di Ferrara, Via Saragat 1, 44122 Ferrara, Italy}
\affil[12]{INFN Sezione di Ferrara, Via Saragat 1, 44122 Ferrara, Italy}
\affil[13]{INAF - OAS Bologna, via Piero Gobetti, 93/3, 40129 Bologna, Italy}
\affil[14]{Dipartimento di Fisica, Università La Sapienza, P. le A. Moro 2, Roma, Italy}
\affil[15]{Instituto de Fisica de Cantabria (IFCA, CSIC-UC), Avenida los Castros SN, 39005, Santander, Spain}
\affil[16]{Dipartimento di Fisica e Astronomia “G. Galilei”, Università degli Studi di Padova, via Marzolo 8, I-35131 Padova, Italy}
\affil[17]{INFN Sezione di Padova, via Marzolo 8, I-35131, Padova, Italy}
\affil[18]{INAF, Osservatorio Astronomico di Padova, Vicolo dell’Osservatorio 5, I-35122, Padova, Italy}
\affil[19]{School of Physics, Indian Institute of Science Education and Research Thiruvananthapuram, Maruthamala PO, Vithura, Thiruvananthapuram 695551, Kerala, India}
\affil[20]{Dipartimento di Fisica, Università degli Studi di Milano, Via Celoria 16 - 20133, Milano, Italy}
\affil[21]{INFN Sezione di Milano, Via Celoria 16 - 20133, Milano, Italy}
\affil[22]{Université Paris-Saclay, CNRS, Institut d’Astrophysique Spatiale, 91405, Orsay, France}
\affil[23]{Institute of Astrophysics, Foundation for Research and Technology – Hellas, Vasilika Vouton, GR-70013 Heraklion, Greece}
\affil[24]{Department of Physics and ITCP, University of Crete, GR-70013, Heraklion, Greece}
\affil[25]{Institut d'Astrophysique de Paris, CNRS/Sorbonne Université, Paris, France}
\affil[26]{School of Physics and Astronomy, Cardiff University, Cardiff CF24 3AA, UK}
\affil[27]{Max Planck Institute for Astrophysics, Karl-Schwarzschild-Str. 1, D-85748 Garching, Germany}
\affil[28]{Excellence Cluster ORIGINS, Boltzmannstr. 2, 85748 Garching, Germany}
\affil[29]{Università di Trento, Dipartimento di Fisica, Via Sommarive 14, 38123, Trento, Italy}
\affil[30]{Kavli Institute for the Physics and Mathematics of the Universe (Kavli IPMU, WPI), UTIAS, The University of Tokyo, Kashiwa, Chiba 277-8583, Japan}
\affil[31]{Université Paris Cité, CNRS, Astroparticule et Cosmologie, F-75013 Paris, France}
\affil[32]{INFN Sezione di Roma, P.le A. Moro 2, 00185 Roma, Italy}
\affil[33]{INFN Sezione di Pisa, Largo Bruno Pontecorvo 3, 56127 Pisa, Italy}
\affil[34]{Institute of Particle and Nuclear Studies (IPNS), High Energy Accelerator Research Organization (KEK), Tsukuba, Ibaraki 305-0801, Japan}
\affil[35]{NASA Goddard Space Flight Center, Greenbelt, MD 20771, USA}
\affil[36]{INFN Sezione Milano Bicocca, Piazza della Scienza, 3, 20126 Milano, Italy}
\affil[37]{Jodrell Bank Centre for Astrophysics, Alan Turing Building, Department of Physics and Astronomy, School of Natural Sciences, The University of Manchester, Oxford Road, Manchester M13 9PL, UK}
\affil[38]{Instituto de Astrofísica de Canarias, E-38200 La Laguna, Tenerife, Canary Islands, Spain}
\affil[39]{Japan Aerospace Exploration Agency (JAXA), Institute of Space and Astronautical Science (ISAS), Sagamihara, Kanagawa 252-5210, Japan}
\affil[40]{The Graduate University for Advanced Studies (SOKENDAI), Miura District, Kanagawa 240-0115, Hayama, Japan}
\affil[41]{Institute of Theoretical Astrophysics, University of Oslo, Blindern, Oslo, Norway}
\affil[42]{INFN Sezione di Bologna, Viale C. Berti Pichat, 6/2 – 40127 Bologna, Italy}
\affil[43]{University of Milano Bicocca, Physics Department, p.zza della Scienza, 3, 20126 Milan, Italy}
\affil[44]{Departamento de Astrofísica, Universidad de La Laguna (ULL), E-38206, La Laguna, Tenerife, Spain}
\affil[45]{The Oskar Klein Centre, Department of Physics, Stockholm University, SE-106 91 Stockholm, Sweden}
\affil[46]{Department of Physics and Center for High Energy and High Field Physics (CHiP), National Central University, Taoyuan City, Taiwan}
\affil[47]{Université Paris-Saclay, CNRS/IN2P3, IJCLab, 91405 Orsay, France}
\affil[48]{Nagoya University, Kobayashi-Masukawa Institute for the Origin of Particle and the Universe, Aichi 464-8602, Japan}
\affil[49]{Okayama University, Department of Physics, Okayama 700-8530, Japan}
\affil[50]{Lawrence Berkeley National Laboratory (LBNL), Computational Cosmology Center, Berkeley, CA 94720, USA}
\affil[51]{University of California, Berkeley, Department of Physics, Berkeley, CA 94720, USA}
\affil[52]{University of California, Berkeley, Space Sciences Laboratory,  Berkeley, CA 94720, USA}
\affil[53]{Suwa University of Science, Chino, Nagano 391-0292, Japan}
\affil[54]{University of California, San Diego, Department of Physics, San Diego, CA 92093-0424, USA}
\affil[55]{SSC Space for the European Space Agency, Camino bajo del Castillo, s/n, Urbanización Villafranca del Castillo, Villanueva de la Cañada, Madrid, Spain}
\affil[56]{Universidad Europea de Madrid, Escuela de Arquitectura, Ingeniería, Ciencia y Computación – STEAM,  28670, Madrid, Spain}
\affil[57]{Space Science Data Center, Italian Space Agency, via del Politecnico, 00133, Roma, Italy}
\affil[58]{Université Grenoble Alpes, CNRS, LPSC-IN2P3, 53, avenue des Martyrs, 38000 Grenoble, France}
\affil[59]{Gran Sasso Science Institute (GSSI), Viale F. Crispi 7, I-67100, L’Aquila, Italy}
\affil[60]{INFN Sezione di Roma2, Università di Roma Tor Vergata, via della Ricerca Scientifica, 1, 00133 Roma, Italy}
\affil[61]{SRON Space Research Organization Netherlands, 2333 CA Leiden, The Netherlands}
\affil[62]{Department of Advanced Energy, Graduate School of Frontier Sciences, the University of Tokyo}
\affil[63]{Tohoku University, Graduate School of Science, Astronomical Institute, Sendai, 980-8578, Japan}
\affil[64]{ILANCE, CNRS – University of Tokyo International Research Laboratory, Kashiwa, Chiba 277-8582, Japan}
\affil[65]{Université Paris Cité, F-75006 Paris, France}
\affil[66]{Istituto Nazionale di Fisica Nucleare–Laboratori Nazionali di Frascati (INFN–LNF), Via E. Fermi 40, 00044, Frascati, Italy}
\affil[67]{Department of Physics, University of Oxford, Denys Wilkinson Building, Keble Road, Oxford OX1 3RH, UK}
\affil[68]{Dpto. de Física Moderna, Universidad de Cantabria, Avda. los Castros s/n, E-39005 Santander, Spain}
\affil[69]{Universitäts-Sternwarte, Fakultät für Physik, Ludwig-Maximilians Universität München, Scheinerstr.1, 81679 München, Germany}
\affil[70]{GRAPPA, Institute for Theoretical Physics Amsterdam, University of Amsterdam, Science Park 904, 1098 XH Amsterdam, The Netherlands}
\affil[71]{Physics and Astronomy Dept., University College London (UCL), UK}
\affil[72]{Department of Physics and Astronomy, University of British Columbia, 6224 Agricultural Road, Vancouver, BC V6T1Z1, Canada}
\affil[73]{The University of Tokyo, Department of Astronomy, Tokyo 113-0033, Japan}
\affil[74]{Department of Economics, Management and Information Science, Onomichi City University, Onomichi, Hiroshima 722-8506, Japan}
\affil[75]{Dipartimento di Fisica, Università di Pisa, Largo B. Pontecorvo 3, 56127 Pisa, Italy}
\affil[76]{NTT, Inc., Otemachi First Square, East Tower, 5-1, Otemachi 1-Chome, Chiyoda-ku, Tokyo 100-8116, Japan}
\affil[77]{Mullard Space Science Laboratory, Department of Space and Climate Physics, University College London, Gower Street, WC1E 6BT, London, UK}
\affil[78]{INAF – Astronomical Observatory of Trieste, Via G. B. Tiepolo 11, 34143 Trieste, Italy}

